A quantum algorithm to count weighted ground states of classical spin Hamiltonians

Ground state counting plays an important role in several applications in science and engineering, from estimating residual entropy in physical systems, to bounding engineering reliability and solving combinatorial counting problems. While quantum algorithms such as adiabatic quantum optimization (AQO) and quantum approximate optimization (QAOA) can minimize Hamiltonians, they are inadequate for counting ground states. We modify AQO and QAOA to count the ground states of arbitrary classical spin Hamiltonians, including counting ground states with arbitrary nonnegative weights attached to them. As a concrete example, we show how our method can be used to count the weighted fraction of edge covers on graphs, with user-specified confidence on the relative error of the weighted count, in the asymptotic limit of large graphs. We find the asymptotic computational time complexity of our algorithms, via analytical predictions for AQO and numerical calculations for QAOA, and compare with the classical optimal Monte Carlo algorithm (OMCS), as well as a modified Grover's algorithm. We show that for large problem instances with small weights on the ground states, AQO does not have a quantum speedup over OMCS for a fixed error and confidence, but QAOA has a sub-quadratic speedup on a broad class of numerically simulated problems. Our work is an important step in approaching general ground-state counting problems beyond those that can be solved with Grover's algorithm. It offers algorithms that can employ noisy intermediate-scale quantum devices for solving ground state counting problems on small instances, which can help in identifying more problem classes with quantum speedups.

==> aqo.tex <==
AQO works by preparing the system in an initial state, which is also a ground state of a Hamiltonian $\hH_x$, and then adiabatically varying the Hamiltonian as $\hH(t) = \alpha(t)\hH_x + \beta(t)\hH_z$ from $t=0$ to $t=T_{\rm AQO}$, with $\alpha(0)=\beta(T_{\rm AQO})=1$ and $\alpha(T_{\rm AQO})=\beta(0)=0$. The most common choices for the initial state and the Hamiltonian are $\ket{\psi(0)} = \bigotimes_{i=1}^{|E|}\ (\ket{0}_i+\ket{1}_i)/\sqrt{2}$ and $\hH_x = -\sum_{i=1}^n\hs_i^x$. In some variations, $\beta$ is fixed while only the ratio $\alpha/\beta$ is varied from $\infty$ to $0$, which leads to the same final state as varying both $\alpha$ and $\beta$ with time. However, as has been observed before~\cite{boixo2013experimental,matsuda2009ground,konz2018uncertain,matsuda2009quantum,king2016degeneracy,mandra2017exponentially,zhang2017advantages,katzgraber2018viewing}, evolving with $\hH_x = -\sum_{i=1}^n\hs_i^x$ leads to exponential suppression of a significant number of classical ground states in the final wave function.

In this section, we will show that the final wave function $\ket{\psi_{\rm target}}$ can be reached in AQO by choosing the initial state as $\ket{\psi(0)}$ in Eq.~(\ref{eqn: Grover}), and the mixing Hamiltonian as
\begin{equation}\label{eqn: Hx}
\hH_x = \frac{U_0-1}{2} = - \ket{\psi(0)}\bra{\psi(0)},
\end{equation}
with $U_0$ in Eq.~(\ref{eqn: Grover}). We will also show that the amplitudes of the wave function in the computational basis, during any time of executing AQO, importance-sample the ground states of $\hH_z$. Both of these facts arise from the relation of $\hH_x$ to $U_0$. Therefore, like Grover's algorithm, the evolution of the wave function is restricted to lie in a smaller, symmetric, subspace than the full Hilbert space, and wave functions in this symmetric space importance-sample the ground states. 
The AQO schedule we consider is $\beta(t)=1-\alpha(t)=t/T_{\rm AQO}$. We analytically derive a lower bound for $T_{\rm AQO}$.

One can implement a discrete-time version of AQO on a circuit by applying the sequence of operators $\prod_{j=1}^{T_{\rm AQO}/\rmd t} \exp(-i\alpha(t_j)\hH_x\rmd t)\exp(-i\beta(t_j)\hH_z\rmd t)$ to $\ket{\psi(0)}$. Figures~\ref{fig: qtm cct}(b) and~(d) show how to implement $\exp(i\alpha\hH_x)$ and $\exp(-i\beta\hH_z)$ for the paw graph in Fig.~\ref{fig: edge covers}. One of the advantages of AQO (and QAOA in Sec.~\ref{subsec: QAOA}) is that it is possible to similarly construct circuits for $\exp(-i\beta \hH_z)$ with polynomially many (i.e., $n^r$ for $n$ qubits) gates for several other practical problems of interest outside NP, even when it is not possible to implement the Grover oracle with polynomially many gates.

If $\hH$ changes adiabatically, the adiabatic theorem guarantees that the final wave function at $t=T_{\rm AQO}$ will be a ground state of $\hH_z$. Specifically, the adiabatic theorem states that~\cite{messiah1964quantum}
\begin{equation}
\expectation{\psi(T_{\rm AQO})} {\hat{P}_\mathcal{G}} \geq 1-\eta^2
\end{equation}
if
\begin{equation} \label{eqn: adia thm}
 \left|\left|\rmd \hat{H}/\rmd t\right|\right| \leq \eta\Delta(t)^2,
\end{equation}
where $\Delta(t)$ is the instantaneous energy difference between the lowest two eigenstates of $\hH(t)$, and $||\cdots||$ denotes operator norm.

Next, we find the spectrum of $\hH(\alpha,\beta) = \alpha\hH_x + \beta\hH_z$, and use this to analyze the scaling of $T_{\rm AQO}$ with the system size for the adiabaticity condition to be satisfied. As an example, Fig.~\ref{fig: edge covers}(b) shows the spectrum of $\hH(\alpha/\beta,1)$ for the edge cover problem on the paw graph.

\subsubsection{Spectrum of $\hH(\alpha,\beta)$.}

The eigenstates of $\hH(\alpha,\beta)$ fall in two kinds. In the first kind, the eigenstates are anti-symmetric combinations $(\sqrt{w(\phi')}\ket{\phi} - \sqrt{w(\phi)}\ket{\phi'})/\sqrt{w(\phi)+w(\phi')}$, with eigenvalue $\lambda=\beta \mathcal{E}_j$, where both $\ket{\phi}$ and $\ket{\phi'}$ are classical states with  classical energy $H_z(\phi)=H_z(\phi')=\mathcal{E}_j$. For every $j$, there are $N_j^{(0)}-1$ such independent eigenstates of $\hH$. The eigenvalues of these states are shown as red lines in Fig.~\ref{fig: edge covers}(b). We will see that the wave function has no overlap with these eigenstates at any time during AQO or QAOA.

The second kind of eigenstates lie in a Hilbert space $\mathcal{H}_S$ spanned by the symmetric basis states
\begin{equation}\label{eqn: basis states}
\ket{\Phi_j} = \frac{\sum_{\phi: H_z(\phi) = \mathcal{E}_j} \sqrt{w(\phi)} \ket{\phi} }{\sqrt{N_j^{(1)}}}.
\end{equation}
Letting $\hat{P}_S$ be the projection operator into $\mathcal{H}_S$, the projected Hamiltonian is $\hH_S(\alpha,\beta) = \alpha\hH_{xS} + \beta\hH_{zS}$, where
\begin{eqnarray} \label{eqn: projected Hamiltonians}
&\hH_{zS} = \hat{P}_S\hH_z\hat{P}_S = \sum_j \mathcal{E}_j\ket{\Phi_j}\bra{\Phi_j}, \nonumber\\
&\hH_{xS} = \hat{P}_S\hH_x\hat{P}_S = - \left(\sum_i \sqrt{N_i^{(1)}}\ket{\Phi_i}\right) \left(\sum_j \sqrt{N_j^{(1)}}\bra{\Phi_j}\right).
\end{eqnarray}

The eigenvalue equation for $\hH_S$ is $\det(\hH_S(\alpha,\beta)-\lambda) = 0$. Note that $\hH_{xS}$ is also a projection operator, like $\hH_x$. Therefore, $\det(\hH_S(\alpha,\beta)-\lambda)$ is at most linear in $\alpha$, and we can use Taylor expansion and Jacobi's formula to write
\begin{eqnarray}\label{eqn: det}
\det(\hH_S(\alpha,\beta)-\lambda) &= \det(\beta\hH_{zS}-\lambda) + \alpha \frac{\rmd \det(\alpha\hH_{xS}+\beta\hH_{zS}-\lambda)}{\rmd\alpha} \nonumber\\
&= \det(\beta\hH_{zS}-\lambda) + \alpha \Tr(\hH_{xS}\ {\rm adj}(\beta\hH_{zS}-\lambda)),
\end{eqnarray}
where adj$(\cdots)$ is the adjugate. Substituting Eq.~(\ref{eqn: projected Hamiltonians}) into Eq.~(\ref{eqn: det}), we obtain
\begin{equation}\label{eqn: det2}
\det(\hH_S(\alpha,\beta)-\lambda) = \prod_j \left( \beta\mathcal{E}_j-\lambda \right) - \sum_k \alpha N_k^{(1)}\prod_{j\neq k} (\beta\mathcal{E}_k-\lambda).
\end{equation}
Then, the eigenvalues $\lambda$ of $\hH_S(\alpha,\beta)$ are given by the implicit algebraic equation
\begin{equation}\label{eqn: eigs}
\sum_j \frac{N_j^{(1)}} {\beta\mathcal{E}_j-\lambda} = \frac{1}{\alpha}.
\end{equation}
For $\alpha, \beta, N_{j-1}^{(1)}, N_j^{(1)} > 0$, the left hand side of this equation is a function of $\lambda$ which monotonically increases from $-\infty$ to $\infty$ as $\lambda$ changes from $\beta\mathcal{E}_{j-1}$ to $\beta\mathcal{E}_j$. Therefore, Eq.~(\ref{eqn: eigs}) has exactly one solution in the range
\begin{eqnarray}\label{eqn: Erange}
& \beta\mathcal{E}_{j-1} \leq \lambda_j \leq \beta\mathcal{E}_j,\ 0<j<m,\nonumber\\
& \beta\mathcal{E}_0-\alpha \leq \lambda_0 \leq \beta\mathcal{E}_0.
\end{eqnarray}
The equalities, $\lambda_j = \beta\mathcal{E}_j$ or $\lambda_{j+1}=\beta\mathcal{E}_j$, hold true only when $\alpha N_j^{(1)}=0$, and $\lambda_0=\beta\mathcal{E}_0-\alpha$ only when $N_0^{(1)}=\mathcal{P}=1$. An interesting special case is when $\hH_x$ and $\hH_z$ commute, in which case $N_j^{(1)}=1$ for exactly one manifold $\mathcal{E}_j$.

\subsubsection{Proof of importance-sampling.}

$\mathcal{H}_S$ is closed under the action of unitaries $\exp(-i\hH_x\alpha)$ and $\exp(-i\hH_z\beta)$, for arbitrary $\alpha$ and $\beta$. The initial state $\ket{\psi(0)}$ [in Eq.~(\ref{eqn: Grover})] lies in $\mathcal{H}_S$, and therefore the instantaneous wave function during any time in AQO lies in $\mathcal{H}_S$. As a result, the instantaneous wave function always importance-samples the ground states $\ket{g}$, leading to Eq.~(\ref{eqn: importance-sampling}) for AQO as well. This is illustrated in Fig.~\ref{fig: main results}(a).

In the adiabatic limit, $\ket{\psi(T_{\rm AQO})}$ lies in $\mathcal{G}$ and in $\mathcal{H}_S$, therefore $\ket{\psi(T_{\rm AQO})} = \ket{\psi_{\rm target}}$.

\subsubsection{Calculating $T_{\rm AQO}$.} 

Naively, one expects that the evolution time $T_{\rm AQO}$ for the adiabaticity condition [Eq.~(\ref{eqn: adia thm})] to be satisfied is $T_{\rm AQO}=\infty$. This naive expectation is because $\hH$ has ground state degeneracy at $t=T_{\rm AQO}$, and therefore the minimum energy gap $\Delta^*$ above $\ket{\psi_{\rm target}}$ is $0$. However, the required $T_{\rm AQO}$ for Eq.~(\ref{eqn: adia thm}) to be satisfied is in fact finite, because the instantaneous wave function always lies in $\mathcal{H}_S$. The energy gap in this subspace is $\Delta = \lambda_1-\lambda_0 > 0$ always if $\mathcal{P}>0$, as shown by Eqs.~(\ref{eqn: eigs}) and~(\ref{eqn: Erange}).

We can lower-bound $T_{\rm AQO}$ for the adiabatic condition to be met, by estimating the minimum value of $\Delta$.  We find from Eq.~(\ref{eqn: det2}) that
\begin{equation}\label{eqn: prod}
\prod_j (\lambda_j - \beta \mathcal{E}_0) = \det(\hH_S(\alpha,\beta) - \beta\mathcal{E}_0) = -\alpha \mathcal{P} \prod_{j\neq0} \beta(\mathcal{E}_j-\mathcal{E}_0).
\end{equation}
Eqs.~(\ref{eqn: Erange}) and~(\ref{eqn: prod}) then result in the inequality
\begin{equation}\label{eqn: inequality}
\alpha\beta\mathcal{P}(\mathcal{E}_1 -\mathcal{E}_0) \leq (\beta\mathcal{E}_0-\lambda_0) (\lambda_1-\beta\mathcal{E}_0) \leq \alpha\beta\mathcal{P} (\mathcal{E}_{m-1}-\mathcal{E}_0).
\end{equation}
Using the relation $|x+y| \geq 2\sqrt{|xy|}$, we then obtain 
$\Delta = \lambda_1-\lambda_0 \geq 2\sqrt{\alpha\beta\mathcal{P}(\mathcal{E}_1-\mathcal{E}_0)}$.
Next, we apply this argument to edge covers, show that the minimum value of $\Delta$ occurs at $\alpha=\alpha^*$ and $\beta=\beta^*$ that polynomially vary with $|V|$ to leading order, and therefore
\begin{equation}
\Delta^* = \Delta(\alpha^*,\beta^*) \gtrsim \sqrt{\mathcal{P}}
\end{equation}
up to polynomial factors in $|V|$.

For $\hH_z$ and $w(\phi)$ in Sec.~\ref{subsec: edge covers}, $\mathcal{E}_0=0, \mathcal{E}_1 = 1$ and $\mathcal{E}_{m-1} = |V|$. The energy gap $\Delta = \lambda_1 - \lambda_0$ is always nonzero except for $\mathcal{P}=0$, which occurs at $q=1$. At this value, $\hH_x$ and $\hH_z$ commute, $N_{m-1}^{(1)}=1$, and the eigenvalues of $\hH_S(\alpha,\beta)$ are $\lambda=\beta|V|-\alpha$ and $\lambda = \beta j$ for $0\leq j < |V|-1$. Then, for the AQO schedule $\alpha=1-\beta$, the energy gap is $\Delta(\mathcal{P}=0)  = |\beta(1+|V|)-1|\Theta(\frac{2}{|V|+1}-\beta) + \beta\Theta(\beta - \frac{2}{|V|+1})$. This is illustrated as the dotted line in Fig.~\ref{fig: edge covers}(b). The minimum energy gap is $\Delta^*=0$ and occurs at $\beta^*= 1/(|V|+1)$. Further, for all $\alpha$ and $\beta$, $\Delta$ always increases with $\mathcal{P}$. This can be seen by differentiating Eq.~(\ref{eqn: eigs}) with $\mathcal{P}$, yielding
\begin{eqnarray}
&\frac{1}{\beta\mathcal{E}_0 - \lambda} + \sum_j \frac{N_j^{(1)}} {(\beta\mathcal{E}_j-\lambda)^2} \frac{\rmd\lambda}{\rmd\mathcal{P}} = \frac{1}{\alpha} \nonumber\\
\Rightarrow & \frac{\rmd\lambda_0}{\rmd\mathcal{P}} < 0, \frac{\rmd\lambda_1}{\rmd\mathcal{P}} > 0, \frac{\rmd\Delta}{\rmd\mathcal{P}} > 0.
\end{eqnarray}
As a result, $\Delta(\mathcal{P} > 0) > \Delta(\mathcal{P}=0)$ at all $\alpha,\beta$. Then, when $\mathcal{P}$ is exponentially small in the number of qubits, $\Delta^*(\mathcal{P}) \sim \sqrt{\mathcal{P}}$ can occur only within an exponentially small range of parameters, $|\beta - 1/(|V|+1)| \lesssim \sqrt{\mathcal{P}}$.

For the edge cover problem, $||\hH_z - \hH_x|| \leq |V|+1, \alpha^*\sim1, \beta^*\sim1/(|V|+1)$. Then, from the adiabatic theorem [Eq.~(\ref{eqn: adia thm})],
\begin{equation}\label{eqn: TAQO}
T_{\rm AQO} \gtrsim \frac{(|V|+1)^2}{4\eta\mathcal{P}}.
\end{equation}
It is reasonable to expect that $\alpha^*$ and $\beta^*$ are not exponentially small for other Hamiltonians too, as long as $\mathcal{E}_1-\mathcal{E}_0$ is not exponentially small in the number of the qubits and $||\hH_z||$ is not exponentially large. Then, for Hamiltonians satisfying these conditions, $\Delta^*\sim\sqrt{P}$ and $T_{\rm AQO} \gtrsim 1/\sqrt{\mathcal{P}}$ to leading order. This is a generalization of the result found in Refs.~\cite{hen2014fast,roland2002quantum,van2001powerful}, extended to importance-sample ground states of general classical Hamiltonians with an arbitrary weight function. Our result in Eq.~(\ref{eqn: TAQO}) has an additional factor $(|V|+1)^2$ arising from $\beta^*$ and $||\hH_z - \hH_x||$ (which were $1/2$ and $2$ respectively in~\cite{hen2014fast,roland2002quantum,van2001powerful}).

\subsubsection{Numerical simulation of AQO for edge covers.}

Figs.~\ref{fig: AQO and qaoa times}(a)-(b) numerically confirm the scaling in Eq.~(\ref{eqn: TAQO}), and the applicability of this asymptotic formula for finite problem sizes. They plot the number of discrete AQO steps $T_{\rm AQO}/\rmd t$ required to reach $\expectation{\psi(T_{\rm AQO})}{P_\mathcal{G}} = 1-\eta^2$ in a simulation of discrete-time AQO of $\hH_z$ in Eq.~(\ref{eqn: Hz}), with discrete time intervals $\rmd t$. In Fig.~\ref{fig: AQO and qaoa times}(a), we plot $T_{\rm AQO}/\rmd t$ for linear graphs with $q=\sin^2(0.3\pi)$, and in Fig.~\ref{fig: AQO and qaoa times}(b), for an ensemble of random graphs of different vertex degrees and different weighting parameters $q$. In both these cases, we find that $T_{\rm AQO}\sim 1/\mathcal{P}$. We did not verify the logarithmic corrections to this scaling, $(|V|+1)^2$, in Eq.~(\ref{eqn: TAQO}). We arbitrarily chose $\eta$ and $\rmd t$ for these plots, but we find the same scaling for any $\eta$ and small enough $\rmd t$.

$T_{\rm AQO}$ in Eq.~(\ref{eqn: TAQO}) scales the same way as $T_{\rm OMCS}$ for fixed $\epsilon$ and $\delta$ [see Eq.~(\ref{eqn: TOMCS})]. Because of the additional counting overhead $T_{\rm count}$ that will be described in Sec.~\ref{subsec: counting}, the total time taken by AQO, $T_{\rm AQO}\times T_{\rm count}$, increases faster with system size than OMCS. Alternative AQO schedules, such as the one in Refs.~\cite{hen2014fast,roland2002quantum,van2001powerful} where the functional forms of $\alpha(t)$ and $\beta(t)$ are optimally chosen, could result in a quadratic speedup of $T_{\rm AQO}$. Rather than pursuing this, we next use a variational algorithm, QAOA, to optimize the quantum evolution. We find potential for a quadratic speedup.

